No Provisioned Concurrency: Fast RDMA-codesigned Remote Fork for Serverless Computing

Serverless platforms essentially face a tradeoff between container startup time and provisioned concurrency (i.e., cached instances), which is further exaggerated by the frequent need for remote container initialization. This paper presents MITOSIS, an operating system primitive that provides fast remote fork, which exploits a deep codesign of the OS kernel with RDMA. By leveraging the fast remote read capability of RDMA and partial state transfer across serverless containers, MITOSIS bridges the performance gap between local and remote container initialization. MITOSIS is the first to fork over 10,000 new containers from one instance across multiple machines within a second, while allowing the new containers to efficiently transfer the pre-materialized states of the forked one. We have implemented MITOSIS on Linux and integrated it with FN, a popular serverless platform. Under load spikes in real-world serverless workloads, MITOSIS reduces the function tail latency by 89% with orders of magnitude lower memory usage. For serverless workflow that requires state transfer, MITOSIS improves its execution time by 86%.

==> bg-new.tex <==
\section{Background and Motivation}
\label{sec:bg}

\subsection{Serverless computing and containers}
\label{sec:bg-serverless}

Serverless computing is an emerging cloud programming paradigm
that allows developers to construct applications efficiently
without explicit resource management. 
Specifically, developers can focus on the core logic of applications,
write the code in managed language runtime like Python
and upload their code as \texttt{functions} to serverless platforms.
The platform automatically runs the functions 
in response to events like invocation requests,
which offers automatic computing resource provision usually by running functions in containers~\cite{openlambda,fn,ibm-fn,sock,aws-fargate,ali-serverless,azure-function,google-serverless,aws-fargate} 
and scales them up or down according to increased or decreased demands.
Hence, serverless computing relieves developers from tedious tasks including provisioning, scheduling, and scaling.
It is also more economical than traditional virtual machine-based solutions
because the serverless providers typically charge in a pay-as-you-go way. 

Serverless computing frameworks widely use containers to execute functions
because they embrace the features of ease-of-deployment, high performance and lightweight resource isolation
with \texttt{cgroup} and \texttt{namespace}.
We focus on container-based serverless computing in this paper. 
%Thus, we mainly focus on container-based serverless computing in this paper.

\subsection{The case for auto-scaling in serverless computing}
\label{sec:auto-scale}

\setlength{\epigraphwidth}{0.42\textwidth}
%\setlength\epigraphrule{0pt}
\renewcommand{\epigraphsize}{\small}

\vspace{-5pt}
\epigraph{``$\dots$for a service to be considered serverless, it \textbf{must scale automatically} with \textbf{no need for explicit provisioning}.''}
{\textit{Cloud Programming Simplified: A Berkeley View on Serverless Computing~\cite{DBLP:journals/corr/abs-1902-03383}}}  
\vspace{-5pt}

\noindent
Auto-scaling---the ability to automatically boot functions on demand 
but does not require explicit resource provisioning---is 
promised by all serverless computing providers, 
including AWS Lambda~\cite{aws-lambda}, Azure Function~\cite{azure-function}, Google Serverless~\cite{google-serverless},
and Alibaba Serverless Application Engine~\cite{ali-serverless}.
It is beneficial in various scenarios. 
From the perspective of programmers, auto-scaling removes their burden on provisioning containers to handle variant workloads.
Meanwhile, burst-parallel serverless applications
such as video processing~\cite{Sprocket,ExCamera} and data analytic~\cite{Locus,DBLP:conf/cloud/ThomasAVP20}
require scaling to thousands of short-lived functions for complex jobs. 
More importantly, load spikes---instantly invoke many instances of a particular function---exist in production serverless workloads~\cite{DBLP:conf/usenix/WangCTWYLDC21,DBLP:conf/usenix/ShahradFGCBCLTR20}.
The top part of Figure~\ref{fig:bg-trace} presents our analysis of two typical functions that undergo spikes in Azure Function's serverless traces~\cite{DBLP:conf/usenix/ShahradFGCBCLTR20}. 
Under spikes, the invocation frequencies can fluctuate to 33,000X within one minute. 
To improve the application performance under such workloads,
serverless frameworks must spawn enough containers to run these functions.
%\tmac{Figure is unclear, e.g., where is a and b? invocation frequencies? how to make the transition to the Key requirement?}

\paragraph{Key requirement: booting containers at multiple machines.}
One machine typically cannot handle the unpredictable spike workloads without sacrificing the performance.
The bottom half of Figure~\ref{fig:bg-trace} quantifies the least machines required to handle each function's workload without stalling their execution,
\eg{waiting for the previous to finish and then start the next. }
The number is estimated by the function execution time and the hardware configurations (\eg{number of CPUs}). 
Function \texttt{660323} and \texttt{9a3e4e} require up to 31 and 10 machines to handle load spikes, respectively. 

\subsection{Auto-scale containers! But at what cost?}
\label{sec:motiv}

\input{motiv-tab.tex}

\paragraph{Cold start cost.}
Booting a container from scratch (\emph{cold start}) is notoriously slow for handling ephemeral serverless workloads~\cite{sock,sand,du2020catalyzer,DBLP:conf/usenix/ShahradFGCBCLTR20,DBLP:conf/cloud/ThomasAVP20,DBLP:conf/asplos/FuerstS21,DBLP:conf/usenix/WangCTWYLDC21,DBLP:conf/cloud/YuLDXZLYQ020,FAASM}: 
the serverless framework needs to not only create a new container
but also initialize the managed runtime of a high-level language. 
For example, the cold start of container may introduce delays of a few seconds in AWS Lambda~\cite{sand}
while initializing the Java runtime for SPECjbb takes around 1.8 seconds~\cite{du2020catalyzer}. 
%preparing a Python package from a remote repository spends about 4.0 seconds~\cite{sock}.

\paragraph{Resource usage cost.}
To alleviate the booting overhead,
various techniques aim to transform \emph{cold start} to \emph{warm start}~\cite{AWS-Lambda-Reuse,openwhisk,sock,sand,DBLP:conf/usenix/ShahradFGCBCLTR20,du2020catalyzer} 
by pre-allocating computing resources, 
as summarized in Table~\ref{tab:motiv-analysis}. 
Caching-based techniques~\cite{AWS-Lambda-Reuse,openwhisk,sock,sand,DBLP:conf/usenix/ShahradFGCBCLTR20},
reuse launched containers for handling subsequent invocations to the same functions. 
To warm start $n$ containers it needs to cache $n$ running instances, 
which inevitably face the trade-off between cold start costs and high resource overhead since the cached containers should match the number of (unpredictable) invocations for possibly many functions.
Some other work leverages the mechanism of fork to 
achieve low-latency function start~\cite{sand,du2020catalyzer} similar as caching, 
which reduces the pre-allocated resource for a particular function $n$ to $1$ per-machine. 
However, fork cannot generalize to remote machines and has scale poorly on a single machine~\cite{DBLP:conf/hotos/BaumannAKR19}. 
Thus, caching and fork require deploying container instances on all the involved machines.

Checkpoint/Restore (C/R) is the only known solution 
that supports remote warm start without pre-deploying resource on the remote machine.
However, 
it is still has an unsatisfactory performance for auto-scaling (demonstrated in \textsection{\ref{sec:motiv-cr}}).


==> caching-table.tex <==
%\textbf{Caching}~\cite{DBLP:conf/sosp/JiaW21,DBLP:conf/asplos/JiaW21,fn,DBLP:conf/usenix/ShahradFGCBCLTR20,openwhisk}
\textbf{\begin{tabular}[c]{@{}c@{}}Caching\\ \cite{DBLP:conf/sosp/JiaW21,DBLP:conf/asplos/JiaW21,fn,sock, DBLP:conf/usenix/ShahradFGCBCLTR20,openwhisk} \end{tabular}}

==> cold-tab.tex <==
\textbf{\begin{tabular}[c]{@{}c@{}}Cold start\\ \cite{docker, DBLP:conf/usenix/WangCTWYLDC21} \end{tabular}}

==> compare-data-share-tab.tex <==
\begin{table*}[t]  
    \centering    
    \vspace{8pt}  
    \begin{minipage}{1\linewidth}
        \caption{\emph{\small{
        A comparison of techniques for sharing data between dependent functions. 
        }}}
        \label{tab:motiv-data-share}
        \end{minipage} %\\[2pt]  
        \ra{1.4}
        \small{            
        \resizebox{.86\textwidth}{!}{%    
        \begin{tabular}{l|ccccc}
            \toprule             
            & \textbf{Fn/OpenWhisk} & \textbf{SAND}~\cite{sand}         & \textbf{Cloudburst}~\cite{cloudburst} & \textbf{Faastlane}~\cite{faastlane}  & \textbf{Remote fork (MITOSIS)} \\ \hline
            \textbf{Local share method}        & Messaging + Database     & Message queue         & Key-value store       & Load/Store                    & Load/Store                     \\
            \textbf{Local performance}         & Low                & Medium                & Medium                & High                          & High                    \\
            \textbf{Remote share method}       & Messaging + Database     & Message queue         & Key-value store       & RPC                           & \red{RDMA}                 \\
            \textbf{Remote performance}        & Low                & Medium                & Medium                & Medium                        & \red{High}                      \\
            \bottomrule
            \end{tabular}
        }
        }
%\\[-15pt]
\end{table*}   

==> cr-tab.tex <==
%\textbf{C/R}~\cite{DBLP:conf/eurosys/WangHW19, du2020catalyzer,DBLP:conf/asplos/Ustiugov0KBG21}
\textbf{\begin{tabular}[c]{@{}c@{}}C/R\\ \cite{DBLP:conf/eurosys/WangHW19, du2020catalyzer,DBLP:conf/asplos/Ustiugov0KBG21,DBLP:conf/eurosys/AoPV22} \end{tabular}}

==> eval-back.tex <==
\section{Evaluation}
\label{sec:eval}

\subsection{Evaluation Environment}

\TODO{xx}

\subsection{Optimizing Application Startup Latency}

\WTX{subsection by WTX}

\paragraph{Methodology} We evaluate our system against docker and runc, with several applications from
ServerlessBench~\cite{DBLP:conf/cloud/YuLDXZLYQ020} (including a Hello-World python application,
a django python application and an image-resize application). We have also evaluated some other applications of image processing~\cite{pillow},
which have been widely deployed in current serverless platforms~\cite{sand, du2020catalyzer}.

\paragraph{Results} \TODO{xx}

\subsection{Improvement Breakdown}

\WTX{
We evaluate the optimization with the image processing application.
As shown in \TODO{xx}, with \sys, the time spent on memory restoration is reduced from \TODO{xx}
to \TODO{xx}. Besides, the overlap of remote fork procedure and isolation environment setup further decrease
the latency of startup.
}

\subsection{Optimizing Application Memory Occupation}

\WTX{subsection by WTX}

\paragraph{Methodology} We evaluate our system with TestCase8 from ServerlessBench~\cite{DBLP:conf/cloud/YuLDXZLYQ020} and
a python hello application. The evaluated python
application will import some libraries, including basic libraries (os, time, math, etc.) and some extra libraries
(django, requests, PIL) if necessary.
We compare the memory usage of the applications launched by our system with that of those launched from scratch.

\paragraph{Results} After the optimization, we can reduce the memory usage from \TODO{xx} to \TODO{xx}. This is because of the fact that
not all the pages allocated during the initialization are used after fork.
As shown in \TODO{xx}, only \TODO{xx} of the pages are touched. Our on-demand technique will allocate the memory on-demand,
thus saving the memory of unused dramatically.

\subsection{Optimizing Parallel Performance}

\WTX{subsection by WTX}

\paragraph{Methodology} We evaluate our system with a simple python application, which will exit after getting a timestamp.
We evaluate the scalability of \sys~against docker and runc.

\paragraph{Results} \TODO{xx}. A latency-throughput figure.

\subsection{End-to-end Evaluation}

We evaluate the performance of \sysfn and compare it with the original system under the bursty workload.
The evaluated application is an image processing function. We create a synthetic trace according to the
dataset from Azure. \TODO{XX} In the first 1 minute, the request rate is steady at 10 RPS. The burst happens
at the 60th second. The request rate increases to 2500 RPS and the request burst lasts for 5 minutes. We
plot the latency of requests and the request rate in 1 timeline figure \TODO{xx}. We have also plot the
CDF figure of the request latency in \TODO{xx}.


==> eval.tex <==
\section{Evaluation} 
\label{sec:eval}

\paragraph{Experimental setup.} 
We conduct all our experiments on a local cluster with 24 machines spread over two racks. 
Each machine has two 12-core Intel Xeon E5-2650 v4 processors and 128GB of DRAM. 
18 machines are further equipped with two ConnectX-4 MCX455A 100Gbps Infiniband RNIC with PCIe 3.0 x16 connected 
to two Mellanox SB7890 100Gbps Switch.  
We use these 18 machines as {\fn} invokers to execute serverless functions and
leave others that do not have RDMA as the load balancers to issue function requests (\textsection{\ref{sec:serverless}}). 

\paragraph{Comparing targets. }
We compare {\sys} to caching and our optimized variants of CRIU~\cite{criu} to start {\fn}'s Docker containers. 
The caching is the vanilla warm start technique in {\fn} while we further integrate CRIU to it. 
The optimizations to CRIU are:
we first apply SOCK's lean container~\cite{sock} and reduce its containerization overhead from 190ms to 10ms, 
similar to {\sys} (\textsection{\ref{sec:orch}}).
Second, we implement on-demand restore mentioned in Replayable Execution~\cite{DBLP:conf/eurosys/WangHW19} to CRIU
and significantly reduce its startup overhead (see Figure~\ref{fig:motiv}). 
Specifically, the comparing targets are:
\textbf{CRIU-tmpfs} provisions the checkpointed file images at local tmpfs, 
serving as the optimal performance of CRIU.
%\textbf{CRIU-copy} first copies the file from remote parent with RDMA before restoring it, 
%reducing the resources for provisioning images (Figure~\ref{fig:overview} (a)).
\textbf{CRIU-remote} stores the images in a well-optimized distributed file system Ceph~\cite{ceph} to prevent resource provision (Figure~\ref{fig:overview} (b)).
For better performance, 
we configure Ceph to store images in-memory and leverage RDMA to accelerate communications~\cite{ceph-rdma}.
Finally, \textbf{Cache(Ideal)} reuses existing containers for all the functions, 
representing the optimal performance of caching (\ie{no startup cost}). 

Without explicit mention, 
we pre-checkpoint the images of CRIU and pre-prepare the descriptor of {\sys}. 
We deploy two kernel threads in {\sys} to handle descriptor fetch and fallback requests. 

\subsection{Microbenchmarks}
\label{sec:micro}

\begin{figure}[!t]
      \hspace{-4mm}
      \begin{minipage}{.48\linewidth}
              \hspace{-1.5mm}
              \includegraphics[scale=1.2,left]{./data/micro/thpt-machine.pdf}
              \end{minipage} \hspace{0.5mm}
              \begin{minipage}{.48\linewidth}
                \includegraphics[scale=1.2]{./data/micro/thpt-latency.pdf} %\\[10pt]
 %             \hspace*{-1mm}
              \end{minipage}  \\[2pt]
              \begin{minipage}{1\linewidth}
                  \caption{\small{ (a) The throughput of starting hello-world containers with the increase of invoker machines. 
                  (b) Throughput-latency when utilizing all (18) invokers. }}
      \label{fig:eval-concurrency}
      \end{minipage} \\[-25pt]
      \end{figure}
\begin{figure}[!t]
  \hspace{-1.5mm}
      \begin{minipage}{.48\linewidth}
          %    \centering
              \hspace{-1mm}
              \includegraphics[scale=1.2,right]{./data/micro/container-time.pdf}
              \end{minipage} %\hspace{-20mm}
              \begin{minipage}{.48\linewidth}
              \vspace{4.5mm}
              \hspace{-5mm}
              \includegraphics[scale=1.2,left]{./data/micro/memory.pdf} %\\[10pt]
              \end{minipage}  %\\[2pt]
              \begin{minipage}{1\linewidth}
                  \caption{\small{(a) 
                  The time for {\fn} load balancers to start various numbers of hello-world functions using 18 invoker machines. 
                  (b) Memory usage for each method for the function on each invoker excluding the nodes for storing the seed and hosting Ceph. }}
      \label{fig:eval-mem}
      \end{minipage} \\[-12pt]
      \end{figure}      

We start evaluating {\sys} with microbenchmarks aiming to answer the following questions: \\[-18pt]
\begin{itemize}[wide, labelwidth=!, labelindent=0pt]
    \item \textbf{\emph{The throughput of remote fork?  }}
    To show how fast can {\sys} fork, 
    we use a container start benchmark to measure how {\sys} scales with the increasing number of invokers in Figure~\ref{fig:eval-concurrency} (a).
    The functions are invoked by the load balancers that 
    start Python hello-world container in Serverlessbench~\cite{DBLP:conf/cloud/YuLDXZLYQ020}.
    We evaluate more complex real serverless functions in \textsection{\ref{sec:eval-app}}. 

    From the figure, we can see that {\sys} can fork more than 10,000 containers with 17 machines (11,002 with total of 18 machines). 
    It's throughput is 2.1X and 14.1X faster than CRIU-tmpfs and CRIU-remote, respectively.
    CRIU-tmpfs is bottlenecked by interacting and parsing images from the tmpfs while 
    CRIU-remote has the costs of distributed filesystem.
    {\sys} also scales linearly with the increasing of invoker machines because it has not saturated the bandwidth of RDMA. 
    The load-balancer can further start 10,000 function containers within 0.86 second, as shown in Figure~\ref{fig:eval-mem} (a).
  \end{itemize} 
\vspace{-15pt}
\begin{itemize}[wide, labelwidth=!, labelindent=0pt]
    \item \textbf{\emph{The latency of remote fork?}} 
    We use the same benchmark but varies the number of load balancer machines, thread and coroutine configuration 
    to measure the latency of function invocation of each method in Figure~\ref{fig:eval-concurrency} (b). 
    All invokers are involved in this experiment. 
    {\sys} can fork 10,000 containers in 858 milliseconds dominated by initializing the sandbox environment,
    but it's still 1.9--26.4X faster than variants of CRIU.
    Note that CRIU has a longer invocation latency than the results in Figure~\ref{fig:motiv} 
    due to the extra create and destroy overhead when integrating to {\fn}. 

    Note that {\sys} achieves 46.4\% peak throughput as Caching(Ideal), 
    which is bottlenecked by pausing and unpausing running containers. 
    This is because {\sys} has extra containerization and remote interaction overheads. 
    Nevertheless, it consumes orders of magnitude smaller memory (described below).     
  \end{itemize}  
\vspace{-15 pt}
  \begin{itemize}[wide, labelwidth=!, labelindent=0pt]
    \item \textbf{\emph{Memory saving.}} 
    {\sys} not only saves the memory for resource provision but also is more cost-effective during runtime. 
    As shown in Figure~\ref{fig:eval-mem} (b), 
    caching needs sufficient running instances (48 Python hello-world containers) to achieve the ideal performance: 
    <1ms startup time and 1,300 throughput per-invoker before running any functions.
    The cost is 261MB memory consumption for this simple function.
    In comparison, CRIU-tmpfs needs to provision a 16MB image while others don't need.
    During runtime, 
    {\sys} also consumes 29.8--46.2\% less memory compared to CRIU
    because it doesn't need to link the CRIU binary.
    Finally, CRIU-remote may take more runtime memory than CRIU-tmpfs 
    due to extra data stored during file transfer process. 
  \end{itemize}  

\begin{figure}[!t]
  \begin{minipage}{.98\linewidth}
          \hspace{0.8mm}  \includegraphics[scale=1.1,center]{./data/loadspike/latency-TC0.pdf}\\[-7pt]
          \includegraphics[scale=1.1,center]{./data/loadspike/mem-TC0.pdf}
          \end{minipage}  \\[2pt]
          \begin{minipage}{1\linewidth}
              \caption{\small{ The average latency (a) and memory consumption (b) of TC0
                under the spikes of \texttt{Func 660323} shown in Figure~\ref{fig:bg-trace}. }}
  \label{fig:eval-spikes-tc0}
  \end{minipage} \\[-20pt]
  \end{figure} 

\subsection{Performance under load spikes}
\label{sec:eval-load-spike}

This section evaluates the performance of {\sys} under load-spikes in real-world serverless workloads (see Figure~\ref{fig:bg-trace}).
Since Azure function only provides the function invocation traces not the detailed function invoked~\cite{DBLP:conf/usenix/ShahradFGCBCLTR20}, 
we evaluate the spikes with two representative functions from ServerlessBench~\cite{DBLP:conf/cloud/YuLDXZLYQ020}:
TC0 is a simple Python hello-world function while TC1 is a complex image processing function. 
The request is generated by triggering the requests according to the time distribution from the trace. 
We only show the results of \texttt{Func 660323} but the others are similar. 
  
\paragraph{Latency reduction. }
Figure~\ref{fig:eval-spikes-tc0} (a) presents the TC0 invocation latencies during load spikes period
while Figure~\ref{fig:eval-cdf-spikes} (a) summarizes the latency CDF. 
The geometric mean of 50$^{th}$ (median) and 99$^{th}$ percentile latency of {\fn}+{\sys} is just 69.2ms and 172.32ms, 
and is 44.55 and 95.24\% smaller than {\fn}, respectively.
Though {\fn} achieves a 65.07\% cache hit rate during this time period, 
it still suffers from significant latency increase due to the queuing effect of previous stalled function requests, 
since the cold start time of TC0 is 1,566X higher than warm start. 
Meanwhile, {\sys} also achieves 59.67 and 87.44\% smaller median latency than CRIU-tmpfs and CRIU-remote, respectively. 
{\sys} is even faster than CRIU-tmpfs because few RDMA is issued for this simple function. 

\iffalse
\begin{figure}[!t]
  \begin{minipage}{.98\linewidth}
          \hspace{0.8mm}  \includegraphics[scale=1.1,center]{./data/loadspike/latency-TC1.pdf}
          \includegraphics[scale=1.1,center]{./data/loadspike/mem-TC1.pdf}
          \end{minipage}  \\[2pt]
          \begin{minipage}{1\linewidth}
              \caption{\small{ The average latency (a) and memory consumption (b) of TC1
                under the spikes of \texttt{Func 660323} shown in Figure~\ref{fig:bg-trace}. }}
  \label{fig:eval-spikes-tc1}
  \end{minipage} \\[-10pt]
  \end{figure} 
\fi  

\begin{figure}[!t]
  \hspace{-4mm}
  \begin{minipage}{.48\linewidth}
%              \vspace{-2mm}
          \includegraphics[scale=1.2,left]{./data/loadspike/cdf-TC0.pdf}
          \end{minipage} \hspace{0.5mm}
          \begin{minipage}{.48\linewidth}
            \includegraphics[scale=1.2]{./data/loadspike/cdf-TC1.pdf} %\\[10pt]
%             \hspace*{-1mm}
          \end{minipage}  \\[2pt]
          \begin{minipage}{1\linewidth}
              \caption{\small{ The CDF of latency of TC0 and TC1 (see Figure~\ref{fig:motiv}) under the spikes of \texttt{Func 660323} shown in Figure~\ref{fig:bg-trace}, 
              respectively.               
              }}
  \label{fig:eval-cdf-spikes}
  \end{minipage} \\[-20pt]
  \end{figure}     

Figure~\ref{fig:eval-cdf-spikes} (b) further present the latency CDF on TC1,
which is similar to TC0. 
Note that we omit the latency variations with time of TC1 due to space limitations. 
The only difference compared to TC0 is that 
{\sys} has a similar performance as CRIU-tmpfs on TC1 because it reads more memory pages through RDMA. 
Nevertheless, we still have 76.35\% shorter function invocation time than CRIU-remote.

\paragraph{Memory saving. }
{\sys} achieves better performance with less memory consumption thanks to the powerful abstraction of remote fork. 
As illustrated in Figure~\ref{fig:eval-spikes-tc0}, 
at 1.6min,
 {\sys} consumes 96\% smaller memory than {\fn} (41M vs. 562M) on TC0. 
TC1 has a similar result so we omit it. 
The caching dominates the extra memory usage of {\fn} 
and it decreases slowly even under low loads.
This is because a cached instance is only evicted by {\fn} after 30 seconds. 
Reducing the cache time would significantly decrease the hit ratio of {\fn}. 
{\sys} also reduces considerable memory compared to variants of CRIU. 
At the same time (1.6min),
{\sys} uses 86\% and 83\% smaller memory than CRIU-tmpfs and CRIU-remote due to less running instances, respectively. 
These results are aligned with our memory analysis (see Figure~\ref{fig:eval-mem} (b)) in microbenchmarks (\textsection{\ref{sec:micro}}). 

\begin{figure}[!t]
  \hspace{-4mm}
  \begin{minipage}{.48\linewidth}
%              \vspace{-2mm}
          \includegraphics[scale=1.2,left]{./data/micro/data-transfer.pdf}
          \end{minipage} \hspace{0.5mm}
          \begin{minipage}{.48\linewidth}
            \includegraphics[scale=1.2]{./data/micro/multi-fork.pdf} %\\[10pt]
%             \hspace*{-1mm}
          \end{minipage}  \\[2pt]
          \begin{minipage}{1\linewidth}
              \caption{\small{ (a) Data share and (b) multi-hops fork performance.     
              }}
  \label{fig:eval-data-share}
  \end{minipage} \\[-30pt]
  \end{figure}

\subsection{Data sharing and multi-hops fork}  

A powerful feature provided by remote fork is transparent data sharing between functions---we pack different 
functions in the same container and thus they can share data via global variable (see Figure~\ref{fig:mfork}). 
Note that the images and descriptors of CRIU and {\sys} are not prepared throughout the evaluations in this section.

\paragraph{Data share performance. }
Figure~\ref{fig:eval-data-share} (a) presents the communication latency for receiving various-sized data
using the data transfer benchmark from ServerlessBench~\cite{DBLP:conf/cloud/YuLDXZLYQ020}. 
Basic {\fn} uses flow~\cite{fn-flow} to pass data between different containers,
which are warmed for {\fn}. 
%We compare it with {\sys} and 
With {\sys} and CRIU-remote, 
the sender can store the data in a global variable, and the receiver only needs to read from it. 
We use rcopy-based CRIU (see Figure~\ref{fig:overview} (a)) as CRIU-remote in this section 
since coordinating with Ceph introduces extra communications 
and is not optimal for evaluations in this secton. 
From the figure we can see
{\sys} is 26.17--66.34\% faster than vanilla {\fn} for paylaods larger than 100KB, thanks to efficient data sharing 
with between via RDMA-based remote fork. 
For smaller payloads, flow piggybacks them in the function requests. 
{\sys} is also 37.89-80.10\% faster than CRIU-remote.
CRIU-remote requires checkpointing the entire image while {\sys} only dumps a minimal container descriptor 
in the sender's DRAM (17.24ms vs. 2.8ms). 
%{\sys} is also more efficient in resuming execution thanks to an OS co-design with RDMA. 

\paragraph{Multi-hops fork performance. }
We evaluate the performance of multi-hops fork by forking a TC0 container sequentially across machines. 
\iffalse
Specifically, 
a single coordinator issues the fork by calling 
\texttt{fork\_prepare}/checkpoint and \texttt{fork\_resume}/restore sequentially. 
\fi
Figure~\ref{fig:eval-data-share} (b) shows the results. 
The latency of fork increases linearly with the number of hops for {\sys} and CRIU-remote as expected. 
{\sys} is 87.74\% faster to finish one hop 
since it doesn't physically checkpoint the image and bypass the overhead of DFS.  

\begin{figure*}[!t]
%  \begin{minipage}{.98\linewidth}
          \begin{minipage}{.72\linewidth}
            \includegraphics[scale=1.25,center]{./data/loadspike/app-comp.pdf}          
          \end{minipage}
          \begin{minipage}{.2\linewidth}
            \vspace{3mm}
          \includegraphics[scale=1.25,center]{./data/loadspike/factor-analysis.pdf}
          \end{minipage}  \\[0pt]
          \begin{minipage}{1\linewidth}
              \caption{\small{ (a) End-to-end function execution time comparisons on FunctionBench~\cite{DBLP:conf/cloud/KimL19}
              and (b) factor analysis of design choices of {\sys}.  
              Note that in (a), the latency is normalized to the latency of CRIU-tmpfs. 
              }}
  \label{fig:end-to-end}
  \end{minipage} \\[-15pt]
  \end{figure*}   

\subsection{End-to-end serverless applications performance}
\label{sec:eval-app}

{\sys} may introduce extra runtime overhead due to additional latency incurred by RDMA,
especially in complex serverless functions. 
To quantify these overheads, 
this section conducts an end-to-end evaluation using real applications from FunctionBench~\cite{DBLP:conf/cloud/KimL19}.
We compare the startup latency of different approaches in Figure~\ref{fig:end-to-end} (a) 
where the latency is normalized to CRIU-tmpfs.
Note that we evaluate two variants of {\sys}: {\sys}-remote reads all pages from parent via RDMA 
while {\sys}-shared uses locally read page to avoid sending extra network requests (\textsection{\ref{sec:vma}}). 

From the figure we can see that {\sys}-remote only incurs up to 1.2X longer execution time than chamelon, 
while others only take 1.01--1.05X more time. 
The increases are mainly due to extra latency of remote fetches, 
since CRIU-tmpfs restores from local DRAM and RDMA's latency is still orders of magnitude high than DRAM~\cite{farm}.
For example, chameleon that renders an HTML page requires reading 2,303 pages from remote. 
Note that CRIU-tmpfs has to pre-prepare function images on each machine while {\sys} only need to prepare one across the cluster. 
Meanwhile, {\sys}-remote reduces the startup latency of CRIU-remote by 25--82\%
where both systems have the same resource provisioned.
Finally, {\sys}-shared has 4--29\% latency reduction compared to CRIU-tmpfs thanks to the more lightweight restore,
\ie{bypass the local filesystem}. 
Sharing pages is common when auto-scaling multiple containers of the same function (\eg{in load spikes of \textsection{\ref{sec:eval-load-spike}}}).

\subsection{Factor analysis}
As illustrated in Figure~\ref{fig:end-to-end} (b),
the base {\sys},
which creates RCQP upon child start can only achieve a peak throughput of 700 containers per second, 
bottlenecked by creating RDMA connections.
Adding DCT (+DCT)  fundamentally addresses this issue.
Finally, sharing pages between containers further improves the peak throughput by 1.1X.

==> fork-tab.tex <==
%\textbf{Fork}~\cite{du2020catalyzer,sock,sand,DBLP:conf/asplos/DuLJXZC22} 
\textbf{\begin{tabular}[c]{@{}c@{}}Fork\\ \cite{du2020catalyzer,sand,DBLP:conf/asplos/DuLJXZC22} \end{tabular}}

==> function-tab.tex <==
\begin{table}[t]  
    \centering    
    \vspace{8pt}  
    \begin{minipage}{1\linewidth}
        \caption{{\small{
        Functions used in the evaluations.
        }}}
        \label{tab:eval-functions}
        \end{minipage} %\\[2pt]  
        \ra{1.4}
        \small{            
        \resizebox{.48\textwidth}{!}{%    
        \begin{tabular}{lccc}
            \toprule                          
            & \textbf{Description} & \textbf{Image size} & \textbf{Working size} \\ \hline
            \textbf{Hello-world} & Print `Hello world'     & \TODO{xx} MB               & \TODO{xx} MB                 \\
            \TODO{xx}                     &                      &                     &                       \\ %\hline
            \bottomrule

            \end{tabular}        
        }
        }
%\\[-15pt]
\end{table}         


==> motiv-tab.tex <==
\begin{table}[t]  
    \centering    
    \vspace{8pt}  
    \begin{minipage}{1\linewidth}
        \caption{{\small{
         Techniques to warm start serverless functions. 
        \textbf{Resource} is the per-machine resource to warm start $n$ invocations of \emph{a particular function}. 
%        \textbf{Container} is the running state (\eg{memory consumption}) of the function container. 
%        The \textbf{warm start} time is measured by a Hello-world serverless function (\textbf{TC0} in Figure~\ref{fig:motiv}).
        The \textbf{warm start} time is measured by TC0 in Figure~\ref{fig:motiv}.
        TC0's cold start time is 783ms with Docker. 
        When the resource is not on the machine, the warm start time becomes \textbf{remote warm start}.
        {\sys} and C/R only need one resource to fast start others at $M$ machines, 
        so the amortized per-machine resource is $1/M$.
        }}}
        \label{tab:motiv-analysis}
        \end{minipage} %\\[2pt]  
        \ra{1.4}
        \small{            
        \resizebox{.48\textwidth}{!}{%    
        \begin{tabular}{l|cccc}  
                \toprule                          
                \textbf{Technique}              & \textbf{\begin{tabular}[c]{@{}c@{}}Resource\\ for warm\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Warm \\ start\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Remote\\ warm start\end{tabular}} \\ \hline
                \input{caching-table.tex}       & $n * container$                                                       &                    < 1ms                                             &            \xmark                                                      \\
                \input{fork-tab.tex}            & $1 * container$                                                       &                      1ms                                             &            \xmark                                                      \\
                \input{cr-tab.tex}              & $(1/M) * image$ $file$                                                &                    14.8ms                                            &                   44ms                                              \\ \hline
                \textbf{\sys}                   & $(1/M) * container$                                                   &                      -                                               &        11ms                                          \\
                \bottomrule
                \end{tabular}%
        }
        }
\\[-15pt]
\end{table}         


==> motiv.tex <==
\subsection{Checkpoint/Restore is inefficient}
%\subsection{\uline{C}heckpoint/\uline{R}estore (C/R) is inefficient}
\label{sec:motiv-cr}

\begin{figure*}[!t]
    \begin{minipage}{.19\linewidth}
        \hspace*{-2.mm}
        \includegraphics[scale=0.8]{./data/motiv/motiv-overall.pdf}        
    \end{minipage}
    \begin{minipage}{.2\linewidth}
        \includegraphics[scale=0.8]{./data/motiv/motiv-overall-1.pdf}        
    \end{minipage}    
    \begin{minipage}{.17\linewidth}
        \vspace{-2.7mm}
        \includegraphics[scale=0.8]{./data/motiv/motiv-criu-checkpoint-bd.pdf}        
    \end{minipage}  
%    \hfill
    \begin{minipage}{.19\linewidth}
        \hspace*{4.mm}
        \includegraphics[scale=0.8]{./data/motiv/motiv-criu-restore-bd-tc6.pdf}        
    \end{minipage}        
    \begin{minipage}{.19\linewidth}
        \hspace*{4.mm}
        \includegraphics[scale=0.8]{./data/motiv/motiv-criu-restore-bd-tc10.pdf}        
    \end{minipage}  \\[-2pt]
    \begin{minipage}{1\linewidth}
        \caption{\small{An analysis of the cost of using \textbf{CRIU}~\cite{criu},
        the state-of-the-art C/R on Linux
         to checkpoint and restore a container from one machine to another. 
        End-to-end latency on two typical functions from ServerlessBench~\cite{DBLP:conf/cloud/YuLDXZLYQ020} (a) \textbf{TC0}, a simple Hello-world function 
        and (b) \textbf{TC1}, a complex image resize function.  
        (c) a breakdown of the checkpoint latencies of the two functions. 
        (d) and (e) are breakdowns of restore and execution time for TC0 and TC1, respectively. 
        We further optimized it with various techniques (see \textsection{\ref{sec:eval}}). %\eg{lean container~\cite{sock} and on-demand restore~\cite{DBLP:conf/eurosys/WangHW19}} (see \textsection{\ref{sec:eval} for more details}). 
        \textbf{CRIU base} stores the images in DRAM while \textbf{CRIU DFS} stores them in Ceph~\cite{ceph}, 
        the state-of-the-art distributed file system (DFS) that supports RDMA.
%        \textbf{Testbed:} The server has two 12-core CPUs and two 100Gbps network cards. 
        }}
        \label{fig:motiv}
    \end{minipage} \\[-15pt]
\end{figure*} 

%% XD: confirmed w/ Mingkai, tmpfs it the fastest file system using DRAM
Figure~\ref{fig:overview} (a) shows using C/R to warm start a container
from one machine (M0) to another (M1).  
The system first selects a previously started container and checkpoints its execution state to image files ({\blue{\ding{182}}}). 
It can be skipped if the M0 already has checkpointed the image. 
M1 can then copy these files to itself ({\blue{\ding{183}}}) and restore the execution accordingly ({\blue{\ding{184}}}). 
Current CRIU implementation loads all memory pages from the files upon restore, 
which is often unnecessary for serverless workloads~\cite{DBLP:conf/eurosys/WangHW19,du2020catalyzer}. 
Hence, we further optimize it with the on-demand restore technique~\cite{DBLP:conf/eurosys/WangHW19}
such that only restore the touched pages ({\blue{\ding{185}}}). 
As illustrated in Figure~\ref{fig:motiv} (d) and (e), 
on-demand restore improves the vanilla CRIU by 22\% and 24\% when restoring from tmpfs for 
TC0 and TC1---two representative functions from ServerlessBench~\cite{DBLP:conf/cloud/YuLDXZLYQ020}, respectively. 
Note that we also optimize its isolation restore (\eg{cgroup}) with SOCK~\cite{sock}, 
otherwise it will dominate the restore (restore isolation in Figure~\ref{fig:motiv} (d), \eg{> 190ms}). 
% TC0: 19 -> 15; TC1: 79.8 -> 60.5. XD: the dominating factor for TC0 is restoring the isolation, while for TC1 is the execution time. 

Though C/R generalizes to a remote setting, it is orders of magnitude slower than caching or fork (see Table~\ref{tab:motiv-analysis})
even with careful optimizations due to the following issues:

\paragraph{Issue\#1. File copy cost. }
Figure~\ref{fig:motiv} (a) and (b) breakdown the overhead of restoring a container from one machine to another. 
For TC0, coping files takes 73\% and 77\% of the total restore and execution time
and for TC1, it consumes 45\% and 52\%, respectively. 
Note that we carefully optimized the copy phase: 
first, the files are stored tmpfs (\ie{in DRAM}) bypassing the slow storage (\eg{SSD});
Second, we copy the file through RDMA. 
Yet, the copy still takes much time. 
The copy overhead increases linearly with the image size, 
and transferring the whole image is usually unneeded due to the on-demand execution nature of typical serverless functions. 
% in-memory states: TC0: 10.2MB TC1: 38MB 

\vspace{-3pt}
\paragraph{Issue\#2. Resource usage cost.}
A naive way to avoid copying files is to pre-deploy these files on all the machines. 
As illustrated in Figure~\ref{fig:motiv} (d) and (e), 
restoring from pre-deployed image on demand (+OnDemand tmpfs) is relative fast: 
it reduces the restore time by 59\% and 65\% (compared with file copy) for TC0 and TC1, respectively.
However, this approach fallbacks to the existing caching technique (\eg{\textsection{\ref{sec:motiv}})
which faces the trade-off of cold start overhead (\ie{copy file}) and high resource overhead.
%because each machine must decide and dedicate resources for image files. 

\vspace{-3pt}
\paragraph{Issue\#3. Access distributed file system cost. }
To reduce resource usage, we can store image files in a distributed file system (DFS), 
as illustrated in Figure~\ref{fig:overview} (b). 
Consequently, each machine can restore from the shared file with minimal local resource usage.
However, DFS introduces higher overhead during container restore ({\blue{\ding{183}}} and {\blue{\ding{184}}} in Figure~\ref{fig:overview} (b))
compared to local filesystem due to the abstractions of remote files. 
As illustrated in Figure~\ref{fig:motiv} (d) and (e), 
using a DFS not only makes the restore process 1.2X and 1.15X slower (+OnDemand tmpfs vs. +OnDemand DFS), 
but also causes 840\% and 81\% slowdowns on the execution for TC0 and TC1, respectively. 
DFS also affects the execution because the memory pages are pulled from it in an on-demand way. 
Note that we have deployed a state-of-the-art DFS (Ceph~\cite{ceph}) backed by fast network (\ie{RDMA}) and stores all files in the DRAM. 

\vspace{-3pt}
\paragraph{Issue\#4. Slow checkpointing.}
Finally, checkpointing a container is slow because it stores all the container's states to files. 
As shown in Figure~\ref{fig:motiv} (c), 
the cost is proportional to the container size (TC0 and TC1 uses 10.2MB and 38MB files, respectively) 
and is dominated by memory checkpointing.
Since checkpointing typically takes tens of milliseconds (\eg{checkpoint TC1 to tmpfs takes 30ms in Figure~\ref{fig:motiv} (c)}),
implementing dynamic checkpointing is inefficient for serverless frameworks.
However, 
fast dynamic checkpoint is crucial to implement the remote fork primitive~\cite{smith1987implementing} that suits serverless well.
We describe it in more details next (\textsection{\ref{sec:overview}}). 


==> old-intro.tex <==
\section{Introduction}

%% introduce serverless
Serverless computing is an emerging cloud computing paradigm widely 
supported by major cloud providers, including but not limited to AWS Lambda~\cite{aws-lambda}, 
Azure Functions~\cite{azure-function}, Google Serverless~\cite{google-serverless},
Alibaba Serverless Application Engine~\cite{ali-serverless}
and Huawei Cloud Functions~\cite{huawei-function}.
One of the key promises of serverless is \emph{auto-scaling}---users only provide serverless 
functions, and serverless platforms automatically provision computing resources 
(\eg{containers\footnote{\footnotesize{We focus on executing serverless functions 
with containers in this paper, which is widely adopted 
by existing platforms~\cite{openwhisk,fn,openlambda,DBLP:conf/asplos/JiaW21}.}}}) 
to execute them. 
On-demand resource provisioning also makes serverless computing economical,
as the platform only bills when functions are executed (no charge for idle time).

%% obstacle to the auto-scaling
However, \emph{coldstart} (\ie{launching a container from scratch}) becomes 
a key challenge for fast auto-scaling, because the start time (>100\,ms) can be orders of 
magnitude higher than the execution time 
for ephemeral serverless functions~\cite{du2020catalyzer,sock,216063}.
\iffalse
However, a single machine has a limited function density and many real-world 
applications require to scale to multiple machines~\cite{DBLP:conf/usenix/ShahradFGCBCLTR20,
DBLP:conf/usenix/WangCTWYLDC21,DBLP:conf/asplos/DuLJXZC22}.
For example, in a trace from Azure Functions~\cite{DBLP:conf/usenix/ShahradFGCBCLTR20},
the call frequency of a serverless function can surge to over 150\,K calls (\texttt{9a3e4e})
per minute, increasing by 33,000$\times$ within one minute (see 
the top part of Figure~\ref{fig:bg-trace}).
Moreover, to avoid stalling numerous newly arriving function calls, 
the platform should immediately launch sufficient containers across 
{multiple machines} (see the bottom part of Figure~\ref{fig:bg-trace}). 
\fi
%% existing solutions
%Reducing the cold start cost 
Accelerating cold start has become a hot research topic~\cite{AWS-Lambda-Reuse,openwhisk,sock,sand,DBLP:conf/usenix/ShahradFGCBCLTR20,
du2020catalyzer, DBLP:conf/eurosys/AoPV22}. 
Most of them transfers the coldstart to a form of `warmstart' by provisioning resources, 
\eg{launching a container from a cached one}. 
However, they require non-trivial resources when scaling functions to 
a distributed setting, 
\eg{each machine should deploy many cached containers}.

Unfortunately, scaling function to multiple machines is common
because a single machine has a limited function capacity. 
Consider the two functions sampled from real-world traces from Azure Functions~\cite{DBLP:conf/usenix/ShahradFGCBCLTR20}. 
The request frequency of a function can surge to over 150\,K calls 
per minute, increasing by 33,000$\times$ within one minute (see 
the top part of Figure~\ref{fig:bg-trace}).
To avoid stalling numerous newly arriving function calls, 
the platform should immediately launch sufficient containers across 
{multiple machines} (see the bottom part of Figure~\ref{fig:bg-trace}). 

Another problem introduced by running functions with containers 
functions cannot directly share states. 
They must pass the states via message passing or cloud storage services,
which has data serialization/de-serialization, memory copies and software storage stack overheads. 
Recent reports shown that these may count up to 95\% of the function execution time~\cite{faastlane, DBLP:conf/cidr/HellersteinFGSS19}. 
Unfortunately, sharing states between functions is common 
in serverless workflows---a mechanism to compose functions into more complex applications~\cite{aws-step, openwhisk-composer}.

\begin{figure}[!t]
	\vspace{-3pt}
	\begin{minipage}{1.\linewidth}
	\includegraphics[scale=1.2]{./data/motiv/motiv-trace-v1.pdf} %\\[-1pt]
	\end{minipage}
	\begin{minipage}{1.\linewidth}
	\hspace{1.5pt}
	\includegraphics[scale=1.2]{./data/motiv/motiv-trace-machine-count.pdf} %\\[1pt]
	\end{minipage}
	\begin{minipage}{1\linewidth}
	\caption{\small{\emph{The timelines of call frequency (top) and %ideal 
	sufficient resource provisioning (bottom) for two serverless functions %with load spikes 
	in a real-world trace from Azure Functions~\cite{DBLP:conf/usenix/ShahradFGCBCLTR20}.
	}}}
	\label{fig:bg-trace}
	\end{minipage} \\[-15pt]
	\end{figure}
	

In this paper, 
we argue that \emph{remote fork}---forking containers 
across machines like a local fork 
 is a promising and powerful primitive 
to enable both efficient function launching (i.e., performance and 
resource provision) and fast direct state sharing. 
First, the fork mechanism has been shown efficient in both performance and 
resource usage for launching containers in the single-machine setting: 
one cached container is sufficient to warmstart numerous containers for %any subsequent 
with 1\,ms time~\cite{sand,du2020catalyzer,DBLP:conf/asplos/DuLJXZC22}. 
By extending the fork mechanism from local to remote, 
one active container on any machine is sufficient to warmstart numerous 
containers efficiently on all machines.
Second, (remote) fork provides transparent intermediate results sharing 
between functions---the code in the container created by the fork can access 
the pre-materialized states of the forked container 
bypassing message passing or cloud storage. 

Existing systems can only achieve a conservative remote fork 
with Checkpoint/Restore techniques~\cite{criu,DBLP:conf/asplos/Ustiugov0KBG21}.
However, we showed that they are not efficient enough for serverless computing,
\ie{even slower than cold start}
due to the cost of checkpointing the parent container into files,
transferring the files to another machine 
and accessing the files through a distributed file system (\textsection{\ref{sec:rfork}}).

\iffalse
Specifically, caching containers~\cite{AWS-Lambda-Reuse,openwhisk,sock,sand,
DBLP:conf/usenix/ShahradFGCBCLTR20} 
allows functions to reuse cached instances without starting them from scratch. 
Yet, each machine must cache sufficient instances for a single function 
to timely handle unpredictable load spikes
\todo{add citations}.\footnote{\footnotesize{\todo{Say something about
the number of instances would be dynamically adjusted by the platform 
according to current workloads.}}}
Sandbox-fork~\cite{du2020catalyzer,sand} leverages the OS fork to launch 
new containers, but each machine still has to deploy multiple dedicated instances 
as forking seeds. 
There is ``no free lunch'' for these resources: 
existing platforms require users to reserve and pay for the provisioned resources
to achieve better performance (\ie{lower response time}), 
for example AWS Lambda Provisioned Concurrency~\cite{aws-pc}.
\fi

\iffalse
The checkpoint/restore-based (C/R) approach~\cite{criu,DBLP:conf/asplos/Ustiugov0KBG21} 
is currently the only way to perform a warm start on a remote machine 
without provisioning resources; it first checkpoints the container to %well-formed? 
an image, then delivers the image through the network or 
a distributed file system (DFS), and finally restores the container from the image.
Unfortunately, when using C/R, \emph{remote start} can be orders of magnitude 
slower than \emph{local start}, even with fast networks (\textsection{\ref{sec:motiv-cr}}). 
First, the container image could be large ({\tbf}\,MB), so that delivering 
the entire image is costly ({\tbf}\,ms). Further, it is also unnecessary
%copying the entire image can be costly and unnecessary
since running serverless functions typically requires a small portion of 
the image (normally less than {\tbf}\%)~\cite{DBLP:conf/eurosys/WangHW19,du2020catalyzer},
such as \todo{XXX}. %checkpointed states
Second, saving the image in a DFS enables on-demand restore, but also incurs 
non-negligible overhead. Further, when restoring memory states from the image, 
it fails to fully utilize \todo{bandwidth or RDMA features??}
of modern networks (\ie{RDMA}).
Finally, checkpointing a container is typically slow ({\tbf}\,ms), 
especially compared to short-lived serverless functions 
(less than {\tbf}\,ms for all functions in \todo{XXX}).
\fi

We present {\sys}, an operating system primitive that provides 
an ultra-efficient \emph{remote fork}.
{\sys} achieves so by deeply co-designing OS 
with modern interconnect (\ie{RDMA}) widely deployed in data-centers. 
The key insight is that an OS can directly access the physical memory on remote machines
via RDMA-capable NICs (RNICs)~\cite{tsai2017lite}, which is extremely fast
thanks to remote Os and CPU bypassing. 
Therefore, {\sys} can map a child container's virtual memory to 
its remote parent container's physical memory
without checkpoint the parent container's memory.  
The child container can further directly 
read the parent states in a \emph{read-on-access} way only using RNIC, 
eliminating additional software 
overheads (\eg{redundant data and file systems}) compared to C/R.

\iffalse
Remote fork is not so new, but existing designs can only achieve a slow implementation based on C/R~\cite{smith1987implementing},
to the best of our knowledge. 
Observing the emergency of remote memory read access (RDMA)---a fast interconnect with remote memory access capabilities, 
we show that it is possible to achieve fast remote fork by imitating local fork with RDMA. 
In particular, OS can directly access another machine's physical memory bypassing the OS and CPU with RDMA-capable NIC (RNIC)~\cite{tsai2017lite}, 
which is extremely fast. 
Thus, we can map a child container's VM to remote parent's physical memory 
and read them with RDMA on-demand in a read-on-access way.
Compared to C/R, this approach bypasses any extra software overhead (\eg{filesystem}). 
\fi

Leveraging RDMA for remote fork poses several new challenges,
including 
(1) fast and scalable RDMA-capable connection establishment, 
(2) safely controlling the access permissions of the parent container's 
exposed physical memory and 
(3) parent container's lifecycle management at scale. 
{\sys} addresses these challenges by 
(1) retrofitting advanced RDMA feature (\ie{DCT~\cite{dct}}),
(2) proposing a new connection-based memory access control method designed for 
remote fork 
and 
(3) co-designing container lifecycle management with the serverless platform. 
Our design illustrates that remote fork is efficient while 
feasible and practical on commodity RNICs for serverless computing. 


\iffalse
However, leveraging RDMA for remote fork poses a significant challenge 
for OS to manage its physical memory as RNICs can access physical memory 
in a CPU/kernel-bypass way. 
Though infrequent, OS may reclaim the physical memory (\eg{``swapped out''}) 
mapped by RNICs for remote machines. 
Traditionally, OS adopts an \emph{active} control model that changes 
the mapping of all processes referencing the page before reclaiming it. 
Unfortunately, the active model is impractical in the context of remote fork,
namely forking thousands of child containers to many remote machines 
from one container
%because a container can be forked to thousands of child containers across machines 
(\eg{Figure~\ref{fig:motiv}}). 

To remedy this issue, {\sys} proposes a \emph{passive} model to manage 
physical memory. Specifically, the parent OS can reclaim physical pages 
mapped by remote child containers without synchronizing with them.
It relies on RNICs to reject future (remote) accesses to these pages.
Thus, child containers can passively detect the reclamation and execute 
a fallback path for correctness.
A straightforward way of realizing this model is to leverage RDMA's 
memory registration~\cite{rdma-manual}. 
However, it is suboptimal for remote fork due to non-trivial registration 
overhead and incompatible issues in the kernel (\textsection{\ref{sec:challenges}}).
To this end, {\sys} further proposes a novel OS mechanism for remote fork,
which leverages dynamic connection authentication feature of advanced 
RDMA transport (DCT)~\cite{dct} to design a \emph{registration-free} 
memory control. 
Finally, RDMA alone is insufficient for fast forking all states of a container. 
Therefore, {\sys} presents several techniques including generalizing single-machine 
lean container~\cite{sock} to a distributed setting
for efficient forked process containerization. \CR{just one tech?}
\fi

\iffalse
%Finally, RDMA alone is insufficient for fast remote fork because re-initializing 
%the sandbox environment is notoriously slow. 
We also introduces techniques including generalizing single-machine lean container~\cite{sock} to a distributed setting. 
\fi

\iffalse
Remote fork is not so new, 
but existing designs are slow because they only achieve a defective implementation with C/R~\cite{smith1987implementing},
to the best of our knowledge. 
Observing the emergency of remote memory read access (RDMA)---a fast interconnect with remote memory access capabilities, 
we propose {\sys}: an OS primitive that realizes ultra-fast remote fork by imitating local fork with RDMA. 
{\sys} extends the OS to support a direct mapping between the child virtual memory (VM) and the (remote) parent physical memory,
whose memory is read via RDMA in an on-demand way well-suited for serverless computing~\cite{DBLP:conf/eurosys/WangHW19, du2020catalyzer} 
and bypasses any extra software overhead compared to C/R. 
Since the RDMA bandwidth is becoming only 2x to 4x slower than local DRAM~\cite{DBLP:conf/osdi/ShanHCZ18}
and its latency is orders of magnitude smaller than the Linux's page fault handler~\cite{DBLP:conf/osdi/RuanSAB20}, 
the RDMA-based remote fork can have a close performance as a local fork. 
We also introduce techniques including fast containerization by generalizing single-machine lean container~\cite{sock}
to a distributed setting and retrofit advanced RDMA transports for fast connection setup and lightweight memory control.

A major challenge addressed by {\sys} is how to safely and efficiently manage the memory exposed to remote machines,
which can be reclaimed by OS routines (\eg{swap}) while remote children concurrently read it in an OS-bypass way. 
Coordinating accesses distributedly requires non-trivial synchronizations between machines, 
which is prohibitive especially when a parent can be forked by thousands of children. 
Though we can leverage RDMA's memory registration to manage the memory without synchronizing with remote peers, 
registering the memory to the RNIC has a non-trivial overhead with limited support in kernel-space RDMA (\textsection{\ref{sec:challenges}}). 
{\sys} solves this problem with a novel mechanism 
that leverages the dynamic connection authentication feature supported in RDMA' advanced transport (\ie{DCT~\cite{dct}}) for lightweight memory management. 
The mechanism provides a similar abstraction as memory registration without physically registering the memory. 
\fi

{\sys} is flexibly implemented on Linux with minor modifications to the kernel. 
For memory safety, we implemented its core part as a loadable kernel module 
using {\tbf}\,LoC Rust code.
It can remote-fork $10,000$ containers on 18 machines in $0.86$ seconds. 
Further, {\sys} is also fully compatible with mainstream container platforms 
(\eg{xx}), making it possible to be integrated with existing container-based 
serverless computing frameworks seamlessly.
To demonstrate the efficiency and efficacy, 
we integrated {\sys} with Fn~\cite{fn}, a popular open-source serverless 
computing framework. For sudden load spikes in real-world serverless workloads, 
{\sys} reduces the median ($50^{th}$) and $99^{th}$ percentile latency of 
spiked function by 44.6\% and 95.2\%, respectively, 
with orders of magnitude lower memory usage. 

%\vspace{1.ex}
\stitle{Contributions}. We make the following contributions: \\[-18pt]
\begin{itemize}[leftmargin=*,leftmargin=10pt,itemindent=0pt]
    \item \textbf{Problem}: An in-depth analysis of the requirements for auto-scaling 
	%containers to multiple machines 
	in serverless computing and the performance-resource provision tradeoff of 
	existing approaches when doing so (\textsection{\ref{sec:bg}}). \\[-18pt]
    \item \textbf{{\sys}}: An RDMA-accelerated OS remote fork primitive 
	that quickly launches containers on remote machines with minimal resource 
	provisioning (\textsection{\ref{sec:rfork}}). \\[-18pt]
    \item \textbf{Demonstration}: An implementation on 
	Linux integrated with Fn (\textsection{\ref{sec:serverless}}) 
	and evaluations on both microbenchmarks and real-world serverless applications 
	%confirm the benefits of {\sys} (\textsection{\ref{sec:eval}}): 
	demonstrate the efficacy of {\sys} (\textsection{\ref{sec:eval}}). 
\end{itemize}

==> overview.tex <==
\section{The {\sys} Operating System}
\label{sec:overview}

\begin{figure*}[!t]     
    \includegraphics[scale=0.98]{./figures/overview.pdf}  \\[2pt]
    \begin{minipage}{1\linewidth}
    \caption{\small{
        The goal of {\sys}: ultra-fast remote fork.
        An overview of approaches to realize it: 
        (a) C/R with only local filesystems (\eg{tmpfs}),  
        (b)  C/R with a fast distributed filesystem (\eg{Ceph~\cite{ceph}}),
        (c) {\sys}. 
    }}
    \label{fig:overview} 
    \end{minipage} \\[-10pt]
\end{figure*}    

\paragraph{Goal: ultra-fast remote fork for serverless computing. }
Remote fork is promising for serverless computing because first, 
it can incur minimal latency and resource provisioning when booting a function to multiple machines. 
%the image is naturally restored on-demand and only one instance is globally required. 
Second, it enables efficient and transparent data sharing between the parent and child containers (\ie{through global variables}),
which is slow in the traditional approach that leverages an external database~\cite{DBLP:conf/cidr/HellersteinFGSS19}.
However, existing systems uses a (defective) remote fork with C/R~\cite{smith1987implementing},
which are inefficient for auto-scaling containers in serverless computing,
as we have analyzed in \textsection{\ref{sec:motiv}}.
{\sys} seeks to provide an ultra-fast remote fork by co-designing OS with modern interconnect technologies. 

\paragraph{Opportunity: hardware-accelerated, globally addressable memory with RDMA. }
Remote Direct Memory Access (RDMA) is a fast and low CPU cost networking feature widely deployed in modern data-centers~\cite{tsai2017lite,DBLP:conf/sigcomm/GuoWDSYPL16,DBLP:conf/nsdi/GaoLTXZPLWLYFZL21}. 
RDMA-capable network cards (RNICs) can directly read the memory of remote machines bypassing the host CPUs (\ie{one-sided RDMA READ}), 
with both low latency (\eg{2$\mu$s}) and high bandwidth (400Gbps~\cite{connect7}). 
We observe that RDMA enables \emph{efficient global addressable memory}: 
given the (physical) address of the remote machine, reading its content can be completely offloaded to the RNIC in the OS~\cite{tsai2017lite}. 
For remote fork, the child machine can directly read the parent's mapped page with RDMA
bypassing DFS (see \textsection{\ref{sec:motiv-cr}}). 

\paragraph{Our approach: imitate local fork with RDMA. }
{\sys} is a new OS primitive that supports forking a container from anywhere. 
%even the it is not on the same machine with the container. 
The core idea is to imitate the execution of a local OS fork with RDMA. 
The key observation is that if each machine's physical address is globally addressable, 
minimal data structures copies,
\eg{registers and page table}---is sufficient to recover a serverless container capable of executing user functions with RDMA.
For example, we can first map the children's VM to remote parent's physical memory with the copied page table. 
Afterward,
the child OS can leverage RDMA to read from the parent in a read-on-access fashion, 
similar to the copy-on-write in local fork. 
\iffalse
Since RDMA's latency is orders of magnitude smaller than Linux's paging mechanism~\cite{DBLP:conf/osdi/RuanSAB20}, 
the remote fork can also have a similar performance as a local fork.
\fi

A remarkable difference compared to C/R techniques is that 
\emph{{\sys} only uses RDMA to restore the children's execution state during runtime, bypasses any software overhead (\eg{interfacting with DFS})
and avoids storing extra local resources (\eg{a local file}))}. 
Hence, it fundamentally avoids the resource provisioning for fast container startup 
and achieve an extremely low-latency boot and execution for serverless computing. 

\input{challenges.tex}

\subsection{Architecture and execution flow}
\label{sec:overview-flow}

\begin{figure}[!t]
    \vspace{-8mm}
%        \centering
        \hspace{-2mm}
        \includegraphics[scale=1.6]{./figures/arch.pdf} \\[-8pt]
        \begin{minipage}{1\linewidth}
        \caption{\small{The architecture of {\sys}. }}
        \label{fig:arch}
        \end{minipage} \\[-25pt]
        \end{figure}

\iffalse
\paragraph{Assumption. }
%{\sys} relies on commodity RDMA-capable NICs but no other specialized hardware.  %% XD: we extend the RNIC
We assume the child machine has the same hardware (\eg{ISA}) and software configurations (\eg{kernel}) as the parents. 
Though machine configurations in datacenters are typically heterogeneous, 
finding a group of machines with a similar configuration is common~\cite{DBLP:conf/nsdi/GaoLTXZPLWLYFZL21, farm}. 
Hence, {\sys} can support efficient remote forks within these groups. 
Finally, we follow the same security model as the containers, \ie{we trust the kernel}. 
\fi
%\tmac{The same hardware and software configurations should be unnecessary actually. RDMA and Linux with {\sys} should be enough?}

\paragraph{Architecture.}
{\sys} follows a decentralized architecture---each machine can fork from others and vice versa.
%\tmac{{\sys} is an OS primitive or mechanism instead of an architecture.}
We extend the kernel with four components shown in Figure~\ref{fig:arch}. 
The fork orchestrator (\textsection{\ref{sec:orch}}) rehearsals the remote fork and provides interfaces to applications (\eg{serverless frameworks}). 
{\sys} uses a network daemon to manage RDMA-capable connections in a scalable manner (\textsection{\ref{sec:network}}). 
Virtual memory (VM) extends the vanilla OS VM subsystems---including page tables and fault handlers (\textsection{\ref{sec:vma}}) 
to support read-on-access remote paging with RDMA. 
Since RDMA alone is insufficient to recover all children's memory states,  
{\sys} leverages RPC to restore them with a fallback daemon hosted on the parent's OS. 

\paragraph{Execution flow.}
As presented in Figure~\ref{fig:overview} (c), {\sys} divides the remote fork into two phases.
First, {\sys} copies the parent container's metadata (\eg{isolation information and page tables}) to a condensed descriptor (\textsection{\ref{sec:orch}}) ({\blue{\ding{182}}}).
Second, the child's OS fetches the descriptor with one-sided RDMA and restores from it, 
similar as the procedure of process copying in a local fork ({\blue{\ding{183}}}).
Note that the restore is more lightweight than C/R because {\sys} can directly recover from the parent's in-memory data structures instead of serialized file content. 
During runtime, {\sys} transparently read the page from parent via one-sided RDMA in an on-demand way ({\blue{\ding{184}}})
since it has mapped the child's memory to the remote parent's physical address. 

%%% legacy contents
\iffalse
\subsection{Design principles of fast remote fork}

We summarize the principle for a fast remote fork for containers as follows: 

\vspace{4pt}
\begin{thmbox}[M]{\textbf{P\#1: OS support for decoupled container. } }
    \TODO{xx} Allow flexible assembly.         
\end{thmbox}


\vspace{8pt}
\begin{thmbox}[M]{\textbf{P\#2: xxx. } }
    \TODO{xx} 
\end{thmbox}

\vspace{8pt}
\begin{thmbox}[M]{\textbf{P\#3: Distributed I/O support as OS abstractions. } }
    \TODO{xx} 
\end{thmbox}

\fi

\iffalse
%% XD: legacy challenges
%\tmac{Miss (a) and (b) in the figure. The caption and the title in figure mismatch.}
%% XD: fixed 
\subsection{Challenges and solutions}
\label{sec:challenges}

We note that recent systems also propose to expose machines' memory to others with RDMA~\cite{DBLP:conf/eurosys/AmaroBLOAPRS20,DBLP:conf/nsdi/GuLZCS17,DBLP:conf/usenix/AguileraACDGNRS18}. 
For example, remote memory paging systems~\cite{DBLP:conf/eurosys/AmaroBLOAPRS20,DBLP:conf/nsdi/GuLZCS17} allow swapping a container to swap in/out its memory page to the remote server memory. 
The access patterns for swap-in pages are similar to the COA we described in \textsection{\ref{sec:overview-flow}}. 
However, their system models---\emph{static RDMA memory management} and \emph{pre-established RDMA connections}
are unsuitable for globally addressable memory required in {\sys}. 
More specifically, 

The biggest challenge we met when imitating the local fork with RDMA is 
\emph{efficiently managing the globally exposed memory}.
Without RDMA, the kernel can trivially control all the references to its physical memory. 
However, RDMA may copy the page tables to the target OS and allow it to access its memory through RDMA. 
As illustrated in Figure~\ref{fig:challenges} (a), 
given a global access key, the target can access any source memory pages with RDMA in a CPU and kernel bypassing way. 

\tmac{So far, C1 and C2 looks more like design-choices instead of two challenges for achieving so-called globally-exposed-memory.}

\paragraph{C\#1. Unsafe when exposing physical memory with RDMA.}
Exposing physical memory as Figure~\ref{fig:challenges} (a) is the most efficient way for remote fork. 
However, it has safety or security issues 
since modern operation systems may dynamically reclaim the process's memory unpredictably, 
\eg{under memory swapping or with Linux kernel samepage merging~\cite{ksm}}. 
When these happen, the forked container can copy incorrect memory content and read an invalid value. 

To remedy this, 
a naive solution is to track all the remote accesses of each memory page in the kernel. 
However, this approach is impractical because significant distributed synchronizations are required to reclaim one memory page,  
because the page can be referenced by many other machines. 
Specifically, the kernel must wait for all the remote machines to agree on not accessing the page before reclaiming. 

\paragraph{C\#2. Inefficient when exposing virtualized memory with RDMA. }
A more feasible solution is to leverage the RDMA to manage the exposed memory. 
In default, RDMA provides a memory registration mechanism that
virtualize the physical memory at the RNIC. 
The OS can control which memory is virtualized. 
As shown in Figure~\ref{fig:challenges} (b), 
to use MR, 
the host first registers the memory to the RNIC.
The RNIC will then generate a MR key for the registered memory. 
To access the registered memory, each RDMA request must pass the correct MR key. 
To reclaim the access permission of a memory page, the OS only needs to deregister the corresponding MR. 

Though MR simplifies exposed memory management, 
it is inefficient because it needs pinning, generating and publishing the memory mapping to the RNIC. 
The cost is proportional to its memory size, 
which can be even larger than checkpoint a container image \TODO{add more detailed data} when used in remote fork. 

The MR also scales poorly for remote fork. 
First, each MR key can only protect one physical page. 
Thus, for each memory page referenced by the container, the RNIC must generate a separate key. 
As a result, it adds a significant amount of metadata. 
Second, registering too many MRs can easily thrash the RNIC's internal cache, causing performance degradation~\cite{tsai2017lite}. 
Finally, MR requires pining the memory at OS--meaning the OS cannot swap the registered memory out. 

\paragraph{Issue\#2.  Lack of protection with global key. }
RDMA provides a global key, which the RDMA can use to access arbitrary physical memory when used in the kernel (see Figure~\ref{fig:challenges} (b)). 
Hence, it bypasses the inefficient and non-scalable memory management of MR (Issue \#1). 
Though efficient, 
this approach leaves all the machine's memory unprotected, and the OS has to track all the remote accesses of each memory page. 
As we have discussed at the beginning of this section, doing so is impractical. 

\paragraph{Solution: replace memory permission checks with network connection permission checks. }
We propose to use the network connection permission checks to constraint the memory accesses of the exposed physical memory. 
The idea is simple: 
the server can shut down a network connection to reject future accesses of the exposed memory, 
since one-sided RDMA is only supported in RDMA's connected transport. 
Thus, we can assign different connections to different portions of VMA to control whether remote nodes can access the memory. 

However, the basic solution only allows coarse-grained memory management since it is costly to create connections dynamically. 
To this end, we further design a fine-grained connection checking primitive based on dynamic connected transport (DCT), 
a less studied but widely supported advanced RDMA feature. 
\XD{needs more details}
\fi

==> rev.tex <==
\gdef\therev{0a5c774}
\gdef\thedate{2022-09-14 00:11:50 +0800}

